On the homotopy theory of Grothendieck \infty-groupoids

We present a slight variation on a notion of weak \infty-groupoid introduced by Grothendieck in Pursuing Stacks and we study the homotopy theory of these \infty-groupoids. We prove that the obvious definition for homotopy groups of Grothendieck \infty-groupoids does not depend on any choice. This allows us to give equivalent characterizations of weak equivalences of Grothendieck \infty-groupoids, generalizing a well-known result for strict \infty-groupoids. On the other hand, given a model category M in which every object is fibrant, we construct, following Grothendieck, a fundamental \infty-groupoid functor \Pi_\infty from M to the category of Grothendieck \infty-groupoids. We show that if X is an object of M, then the homotopy groups of \Pi_\infty(X) and of X are canonically isomorphic. We deduce that the functor \Pi_\infty respects weak equivalences.

==> macros.tex <==
\makeatletter

% newtheorem

\theoremstyle{plain}
\newtheorem*{thm*}{Theorem}
\newtheorem{thm}[subsection]{Theorem}
\newtheorem{prop}[subsection]{Proposition}
\newtheorem{lemma}[subsection]{Lemma}
\newtheorem{coro}[subsection]{Corollary}
\newtheorem{conj}[subsection]{Conjecture}

\theoremstyle{definition}
\newtheorem{paragr}[subsection]{}
\newtheorem{ex}[subsection]{Example}
\newtheorem{exs}[subsection]{Examples}
\newtheorem{rem}[subsection]{Remark}
\newtheorem{rems}[subsection]{Remarks}

\newenvironment{tparagr}[1]%
  {\begin{paragr} \textbf{#1.}}
  {\end{paragr}}

%\renewcommand\thesubsection{\thesection.\arabic{subsection}}
%\let\tparagr\subsection

% présentation
\newcommand\ndef[1]{\emph{#1}}
\newcommand\zbox[1]{\makebox[0pt][l]{#1}}
\newcommand\pbox[1]{\zbox{\quad#1}}

\newcommand\nvepsilon\epsilon

\newcounter{myenumerate}
\newenvironment{myenumerate}{%
  \setcounter{myenumerate}{0}%
  \renewcommand\item{%
  \par
  \refstepcounter{myenumerate}%
  \themyenumerate. }}{}

\newenvironment{myenumeratep}{%
  \setcounter{myenumerate}{0}%
  \renewcommand\item{%
  \par
  \refstepcounter{myenumerate}%
  {\rm (\themyenumerate)} }}{}

\newenvironment{myitemize}{%
  \renewcommand\item{%
  \smallskip
  \par
  $\bullet$ }}{\par}
 
\renewcommand\epsilon\varepsilon 

\newcommand\bs\backslash

% théorie des catégories
\newcommand\op{\mathrm{o}}
\newcommand\pref[1]{\widehat{#1}}
\DeclareMathOperator{\Hom}{\mathsf{Hom}}
\DeclareMathOperator{\Homi}{\underline{\mathsf{Hom}}}

%
\newcommand\timesh{\times^{\mathrm{h}}}

% 2-flèches
\newcommand{\Rtarrow}{\operatorname{\Rightarrow}\limits}

% infini-catégories
\newcommand{\oo}{$\infty$\nobreakdash}

% noms de catégories
\newcommand{\Dlt}{\Delta}
\newcommand{\Th}{\Theta}
\newcommand{\Thtld}{\widetilde{\Theta}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\Gn}[1]{\mathbb{G}_{#1}}
\newcommand{\Thz}{\Th_0}
\newcommand\Set{{\mathcal{S} \mspace{-2.mu}{et}}}
\newcommand{\Top}{{\mathcal{T}\hskip -2.5pt op}}
\newcommand{\Cat}{{\mathcal{C} \mspace{-2.mu}{at}}}
\newcommand{\Hot}{\mathsf{Hot}}
\newcommand{\Ho}{{\operatorname{\mathrm{Ho}}}}
\newcommand\Mod[1]{{\operatorname{\mathrm{Mod}}(#1)}}

\newcommand{\@Gpd}[3]{{\operatorname{\text{$#1$}{\mathcal{#2G} \mspace{-0.5mu}{pd#3}}}}}
\newcommand{\gpd}{{\@Gpd{}{}{}}}
\newcommand\Gpd\gpd
\newcommand{\ngpd}[1]{{\@Gpd{#1-}{}{}}}
\newcommand{\wgpd}{{\@Gpd{\infty-}{}{}}}
\newcommand\wgpdC[1]{{\wgpd_{#1}}}

\newcommand\W{\mathcal{W}}
\newcommand{\C}{\mathcal{C}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\AAM}{(A \amalg A)\backslash\mathcal{M}}
\newcommand{\MBB}{\mathcal{M}/(B \times B)}
\newcommand{\MBBp}{\mathcal{M}/(B' \times B')}
\newcommand{\MXX}{\mathcal{M}/(X \times X)}
\renewcommand{\AA}{A \amalg A}
\newcommand{\BB}{B \times B}
\newcommand{\XX}{X \times X}
\newcommand{\N}{\mathcal{N}}
\renewcommand{\P}{\mathcal{P}}

% morphismes de catégories
\newcommand\ceps[1]{{\varepsilon^{}_{#1}}}
\newcommand\cepsp[1]{{\varepsilon'_{#1}}}
\newcommand\id[1]{{1^{}_{#1}}}

% tableaux des dimensions
\newcommand\tabdimi[1][n]{%
{\left(
\begin{matrix}
i_1 && i_2 && \cdots && i_{#1} \cr
& i'_1 && i'_2 & \cdots & i'_{{#1}-1}
\end{matrix}
\right)}}
\newcommand\tabdimj[1][n]{%
{\left(
\begin{matrix}
j_1 && j_2 && \cdots && j_{#1} \cr
& j'_1 && j'_2 & \cdots & j'_{{#1}-1}
\end{matrix}
\right)}}
\newcommand\tabdim{{\tabdimi{}}}
\newcommand\tabdimijk{%
\left(
\begin{smallmatrix}
i & & j \cr
& k
\end{smallmatrix}
\right)}

%% Top

% objets de Top
\newcommand{\eDtop}[1]{\partial\mathbf{D}_{#1}}
\newcommand{\Dtop}[1]{\mathbf{D}_{#1}}
\newcommand{\Stop}[1]{\mathbf{S}^{#1}}

% morphismes de Top
\newcommand{\Topt}[2][\@empty]{%
  \ifx\@empty#1
  \hbox{\boldmath$\tau$}_{#2}%
  \else
  \hbox{\boldmath$\tau$}_{#1}^{#2}%
  \fi
}
\newcommand{\Tops}[2][\@empty]{%
  \ifx\@empty#1
  \hbox{\boldmath$\sigma$}_{#2}%
  \else
  \hbox{\boldmath$\sigma$}_{#1}^{#2}%
  \fi
}

% extensions globulaires
\newcommand\CHAb{C[h_A]^\flat}
\newcommand\CHAd[2]{{#1}[h_{#2}]}
\newcommand\CHA{\CHAd{C}{A}}
\newcommand\glcomp[1]{\overline{#1}}

% morphismes de G
\newcommand{\Glt}[2][\@empty]{%
  \ifx\@empty#1
    t_{#2}%
  \else
    t_{#1}^{#2}%
  \fi
}
\newcommand{\Gls}[2][\@empty]{%
  \ifx\@empty#1
    s_{#2}%
  \else
    s_{#1}^{#2}%
  \fi
}

% morphismes de oo-groupoïdes
\newcommand{\Glk}[2][\@empty]{%
  \ifx\@empty#1
    k_{#2}%
  \else
    k_{#1}^{#2}%
  \fi
}

\newcommand{\Glkp}[2][\@empty]{%
  \ifx\@empty#1
    k'_{#2}%
  \else
    k_{#1}^{'#2}%
  \fi
}

\newcommand{\Glw}[2][\@empty]{%
  \ifx\@empty#1
    w_{#2}^{}%
  \else
    w_{#1}^{#2}%
  \fi
}

\newcommand{\comp}{\operatorname{\ast}\limits}

\newcommand\tildeh[1][\@empty]{%
\ifx\@empty#1
  \sim%
\else
  \sim_{#1}%
\fi
}

\newcommand\PI\varpi

% objets de Theta
\newcommand{\Sn}[1]{{\mathrm{S}^{#1}}}
\newcommand{\Dn}[1]{{\mathrm{D}_{#1}}}
\newcommand{\Dnp}[1]{{\mathrm{D}'_{#1}}}
\newcommand{\eDn}[1]{{\partial\mathrm{D}_{#1}}}
\newcommand{\amalgd}[1]{\amalg^{}_{\Dn{#1}}}

% morphismes de Theta
\newcommand{\Tht}[2][\@empty]{%
\ifx\@empty#1
\tau_{#2}^{}%
\else
\tau_{#1}^{#2}%
\fi
}
\newcommand{\Ths}[2][\@empty]{%
\ifx\@empty#1
\sigma_{#2}^{}%
\else
\sigma_{#1}^{#2}%
\fi
}
\newcommand{\Thkp}[2][\@empty]{%
\ifx\@empty#1
\kappa'_{#2}%
\else
\kappa_{#1}^{'#2}%
\fi
}
\newcommand{\Thk}[2][\@empty]{%
\ifx\@empty#1
\kappa_{#2}^{}%
\else
\kappa_{#1}^{#2}%
\fi
}
\newcommand{\Thnp}[2][\@empty]{%
\ifx\@empty#1
\nabla'_{#2}%
\else
\nabla_{#1}^{'#2}%
\fi
}
\newcommand{\Thn}[2][\@empty]{%
\ifx\@empty#1
\nabla_{#2}^{}%
\else
\nabla_{#1}^{#2}%
\fi
}
\newcommand{\Thw}[2][\@empty]{%
\ifx\@empty#1
\Omega_{#2}^{}%
\else
\Omega_{#1}^{#2}%
\fi
}

% fin
\makeatother

